Scalable Optimal Deployment in the Cloud of Component-based Applications using Optimization Modulo Theory, Mathematical Programming and Symmetry Breaking

The problem of Cloud resource provisioning for component-based applications consists in the allocation of virtual machines (VMs) offers from various Cloud Providers to a set of applications such that the constraints induced by the interactions between components and by the components hardware/software requirements are satisfied and the performance objectives are optimized (e.g. costs are minimized). It can be formulated as a constraint optimization problem, hence, in principle the optimization can be carried out automatically. In the case the set of VM offers is large (several hundreds), the computational requirement is huge, making the automatic optimization practically impossible with the current general optimization modulo theory (OMT) and mathematical programming (MP) tools. We overcame the difficulty by methodologically analyzing the particularities of the problem with the aim of identifying search space reduction methods. These are methods exploiting:(1) the symmetries of the general Cloud deployment problem, (2) the graph representation associated to the structural constraints specific to each particular application, and (3) their combination. An extensive experimental analysis has been conducted on four classes of real-world problems, using six symmetry breaking strategies and two types of optimization solvers. As a result, the combination of a variable reduction strategy with a column-wise symmetry breaker leads to a scalable deployment solution, when OMT is used to solve the resulting optimization problem.

==> preliminaries.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%% sec: preliminaries %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Solution}\label{sec:solution}
In this section, we present our solution approach for solving the COP introduced in Section~\ref{sec:problem}. A natural strategy would be to encode it as an OMT problem and use state of the art OMT tools (e.g. Z3~\cite{10.1007/978-3-540-78800-3_24}, OptiMathSat~\cite{10.1007/978-3-319-21690-4_27}, Symba~\cite{DBLP:conf/popl/LiAKGC14}) for obtaining automatically the solution (see Section~\ref{sec:sec:SMTOMT}). However, due to huge computational requirement, it could not be
carried out in practice. \textcolor{red}{Thus, we proceeded as follows ...:}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% sec: Satisfiability and Optimization Modulo Theories %%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Satisfiability and Optimization Modulo Theories}\label{sec:SMTOMT}
SMT solving is an extension of satisfiability (SAT) solving by introducing the possibility of stating constraints in some expressive theories, for example arithmetic, data structures, bit-vector expressions and their valid combinations. The idea behind SMT solving is that, given a formula in a certain theory, this is translated into a propositional formula. This is checked for satisfiability using a SAT solver. If unsatisfiability can not be deduced, then a candidate model (variables assignment) is fed to the theory solver. If this candidate model makes the initial formula true, SAT is returned meaning that the initial formula is true for the respective model. If SAT can not be deduced then the theory solver backtracks trying another candidate model. This process is repeated until no more candidate models are found.
%\begin{figure}[h!]
%\centering
%\includegraphics[width=0.4\textwidth,height=0.2\textheight]{SMTApproach.png}
%\caption{SMT Approach}
%\label{fig:SMT}
%\end{figure}

For our problem, we needed a SMT solver which exhibits optimization features, the so-called \emph{Optimization Modulo Theories (OMT) solvers}. We did not have too many options in this regard:
\begin{inparaenum}[\itshape (i)\upshape]
	\item OptiMathSAT \cite{10.1007/978-3-319-21690-4_27} uses an inline architecture in which the SMT solver (MathSAT5\footnote{\url{http://mathsat.fbk.eu}}) is
	run only once and its internal SAT solver is modified to handle the search for the optima, 
	\item Symba \cite{DBLP:conf/popl/LiAKGC14} and $\nu Z$ \cite{DBLP:conf/tacas/BjornerPF15} both are based on an offline architecture in which the SMT solver Z3 \cite{10.1007/978-3-540-78800-3_24} is incrementally called multiple times as a black-box.
\end{inparaenum}
%\textcolor{red}{This just for us, to be commented: Different optimization solvers based on SMT (there are only 3 that I found and I think are  the only one since I checked related work from 2017) differently the problem, so there is no unique algorithm. I presented some details of the $\nu Z$ the solver that we used, but not completely since if we would have a COP with soft constraints then the solver behaves internally different.}
Since Symba is not actively maintained and, in our experiments, $\nu Z$ outperformed OptiMathSAT \cite{Erascu_SMT_2019}, in this paper we will use $\nu Z$. It is built on top of the mature SMT solver Z3, it was widely used in various application domains and offers a Python API. It takes as an input SMT formulas (constraints and objectives) which are rewritten and simplified to Pseudo-Boolean Optimization (PBO) constraints. The PBO solver implements a wide range of methods for simplification and generating conflicting clauses, and compiling them into small sorting circuits. At the heart of the tool lies the dual simplex algorithm which is also used to prune branches. 

We \emph{formalized} the problem in quatifier-free linear integer arithmetic since the state-of-the-art OMT tools offer efficient decision procedure for this kind of theory. The timing results are presented in Table \ref{tab:ComparisonVariableEncoding}. For solving the problem, we needed to know in advance the maximum number of VMs that the problem requires. This is not a fixed parameter in our approach, but is computed using the structural constraints which involve number of instances \textcolor{red}{and conflicts???} (see \texttt{init\#VMs} in the tables). %This preprocessing step is not computationally expensive because it solves a constrained optimization problem with a number of variables equal to the number of components.

We studied the scalability of the OMT tools for the case studies from Section \ref{sec:casestudies} from two perspectives: number of VMs offers, respectively number of deployed components.  For \textit{Secure Web Container}, \emph{Secure Billing Email} and \textit{Oryx2} applications, we considered up to 500 CPs offers. Additionally, for the \emph{Wordpress} application, we considered the number of instances of Wordpress component to be deployed. The set of offers was crawled from the Amazon CPs offers list. 

All tests in this paper were done on an MacBook Pro with the following configuration: 3.1~GHz dual-core Intel Core i5 using Z3 version 4.8.7. In Table \ref{tab:ComparisonVariableEncoding}, we included only those results for which we obtained a result in 40 minutes timeframe, as this was the time limit in the SMT-COMP'19\footnote{\url{https://smt-comp.github.io/2019/}}. \textcolor{red}{One can observe that $\nu Z$ does not scale well for high number of VMs offers and components, while OptiMathSAT even for small number of offers. From the logs, we observed that later reached many times the minimum but failed to prove it.} 
\begin{table}[h]
	\centering
	\scriptsize
	\caption{Scalability tests for $\nu$Z/OptiMathSAT tools. Time values are expressed in seconds. (at most 40 minutes = 2400 secs)}
	\begin{tabular}{|c|c|c|c|c|c|c|c|} 
		\hline
		\multirow{2}{*}{\textbf{Problem} } & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}} init\#\\VMs \end{tabular}}} & \multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}\#offers \\ = 20 \end{tabular}}} & \textbf{ \begin{tabular}[c]{@{}c@{}}\#offers \\ = 40 \end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}} \#offers \\ = 100 \end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}} \#offers \\ = 250 \end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}} \#offers \\ = 500 \end{tabular}} \\ 
		\cline{3-8}
		&  & $\nu$Z  & \begin{tabular}[c]{@{}c@{}}Opti\\ MathSAT \end{tabular} & $\nu$Z  & $\nu$Z  & $\nu$Z  & $\nu$Z  \\ 
		\hline
		\textbf{Oryx2}  & 11 & \textbf{6.62} & 59.7 & 8.74 & 21.84 & 73.56 & 193.69 \\ 
		\hline
		\begin{tabular}[c]{@{}c@{}} \textbf{Secure Web} \\ \textbf{Container} \end{tabular} & 6 & 0.27 & - & 0.45 & 1.8 & 8.56 & 35.25 \\ 
		\hline
		\begin{tabular}[c]{@{}c@{}} \textbf{Secure Billing} \\ \textbf{Email} \end{tabular} & 6 & 0.27 & - & 0.45 & 1.8 & 8.56 & 35.25 \\ 
		\hline
		\begin{tabular}[c]{@{}c@{}}\textbf{Wordpress} \\ \textbf{min\#inst = 3} \end{tabular} & 10 & 16.39 & - & 120.84 & 1444.12 & - & - \\ 
		\hline
		\begin{tabular}[c]{@{}c@{}}\textbf{Wordpress} \\ \textbf{min\#inst = 4} \end{tabular} & 10 & 16.39 & - & 120.84 & 1444.12 & - & - \\ 
		\hline
		\begin{tabular}[c]{@{}c@{}}\textbf{Wordpress} \\ \textbf{min\#inst = 5} \end{tabular} & 12 & 775.7 & - & - & - & - & - \\ 
		\hline
		\begin{tabular}[c]{@{}c@{}}\textbf{Wordpress} \\ \textbf{min\#inst = 6} \end{tabular} & 13 & 3516.19???? & - & - & - & - & - \\
		\hline
	\end{tabular}
	\label{tab:ComparisonVariableEncoding}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% sec: Symmetries %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Symmetries and symmetry breakers}\label{sec:symmetries}

From the results in Section \ref{sec:SMTOMT}, we conclude that the naive application of general OMT techniques is not sufficient to solve realistic Cloud deployment applications. This is due to the large solutions space, which, however, might contain equivalent solutions. Therefore, in order to reduce the search space, in this section:
\begin{enumerate}
	\item we describe systematically row and column symmetries for our problem, and	
	\item we come up with some symmetry breakers to eliminate some symmetries described, in order to speed-up the computations.
\end{enumerate}

First we introduce some theoretical notions. A \emph{matrix model} is a constraint program that contains one or more matrices of decision variables. %The problem introduced in Section \ref{sec:problem} is a matrix model, where the decision variable $A$ expresses the fact that a component is assigned, or not, to a VM.  
\emph{Symmetries} in constraints satisfaction/optimization problems, in general, and in matrix models, in particular, are a key problem since search can revisit equivalent states many times. Elimination of the equivalent states, problem known as \emph{symmetry breaking}, has, most of the times, a positive impact in the computation time of the problem solution process. For matrix models, symmetry often occurs because groups of objects within a matrix are identical. 
%For our problem, VMs having the same type are considered identical \textcolor{red}{We should define somewhere what VMType means: a VM which is characterized uniquely by CPU, Mem, Sto, Price}. We can therefore permute any two VMs as long as they have the same type. 
That is, we can permute any two rows/columns of the assignment matrix. This leads to \emph{row/column symmetries}. A row/column symmetry of a bidimentional matrix is a bijection between the variables of two of its rows/columns that preserves solutions and non-solutions. Two rows/columns are identical if their variables are pairwise identical due to a row/column symmetry. A matrix model has \emph{row/column symmetry} iff all the rows (columns) of one of its matrices are \emph{indistinguishable}. A matrix model has \emph{partial row/column symmetry} iff strict subset(s) of the rows
(columns) of one of its matrices are \emph{indistinguishable}. A \emph{symmetry class} is an
equivalence class of assignments, where two assignments are equivalent if there is
some symmetry mapping one assignment into the other. %(In group theory, such equivalence classes are referred to as orbits.)
%Definition already introduced and it's basically the same: In order to deal with symmetries, one must first define what they are. We borrow the definition from \cite{DBLP:conf/cp/FlenerFHKMPW02}, namely ''a symmetry is a bijection on decision variables that preserves solutions and non-solutions. Two variables are indistinguishable if some symmetry interchanges their roles in all solutions and non-solutions.''

%According to \cite[Chapter~10]{DBLP:reference/fai/2}, the type of symmetries introduced above are \emph{solution symmetries}, that is \emph{properties of the solution set}.
%there are two types of symmetries:
%\begin{itemize}
%	\item \emph{problem symmetries} are properties identified in the problem formalization without solving it;
%\end{itemize}

%\noindent In this paper, we deal with \emph{solution symmetries} defined by \cite{DBLP:journals/njc/BrownFP96}: ``A symmetry is a permutation that leaves invariant the set of solutions sequences to a problem.'' For example, if $[2.808, 2.808, 2.808, 2.808, 1.6, 0]$ is a solution then also $[2.808, 2.808, 2.808, 1.6,  0, 2.808]$ is a solution. Equivalently, if $$
%\sigma_1 = \left( \begin{array}{rrrrrr}
%1 & 2 & 3 & 4 & 5 & 6  \\
%1 & 2 & 3 & 4 & 5 & 6
%\end{array}\right) $$ \noindent is the identity symmetry then $$
%\sigma_2 = \left( \begin{array}{rrrrrr}
%1 & 2 & 3 & 4 & 5 & 6  \\
%1 & 2 & 3 & 6 & 4 & 5
%\end{array}\right) $$ \noindent is also a symmetry. Hence, it suffices to consider only $\sigma_1$ and eliminate $\sigma_2$, process known as \emph{symmetry breaking}. Its benefit is the reduction of the search space. Its goal is to never explore two states which symmetric since they are equivalent and the result will be the same.

Needless to say, symmetries depend also on the way the constrained optimization/satisfaction problem is formulated.

Paper \cite[Chapter~10]{DBLP:reference/fai/2} categorized symmetry breaking as follows: 
\begin{itemize}
	\item \emph{Static symmetry breaking} adds the so-called symmetry breaking constraints before search starts, hence making some symmetric solutions unacceptable while leaving at least one solution in each symmetric equivalence class.
	\item \emph{Dynamic symmetry breaking} breaks symmetry dynamically during search, adapting the search
	procedure appropriately.
\end{itemize}

In this paper we use \emph{static symmetry breaking}. 

The symmetries of the Cloud resource provisioning problem as introduced in Section \ref{sec:problem} are described below. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% sec: Column symmetries %%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Column symmetries}\label{sec:colsym}
Consider the decision variable $\emph{vmType}$.  A solution of $\emph{vmType}$ is unique up to permutations of its elements. Moreover, if to its elements $\emph{vmType}_i$, for $i=\overline{1,M}$, are assigned the same value then they are indistinguishable.
\begin{description}
	\item[Type $1$ symmetry] Two or more VMs are undistinguishable if they have the same type. One type of symmetry breakers are the following formulae:
	\begin{alignat*}{2}
	& \emph{VP}_k \ge \emph{VP}_{k+1} , & &\quad \text{for all } k=\overline{1,M-1}
	\end{alignat*}
	There are also other types of symmetry breakers which can be used, for example, those involving the hardware characteristics (e.g. CPU, memory, storage) of a VM type. However, the symmetry breaker must involve only one of the hardware characteristics. This is due to the fact that there can not be imposed a lexicographic order on the elements of two distinct elements of $\emph{vmType}$. An exemplification in this sense are the following two VM types as crawled from the Cloud Providers site:
	\begin{verbatim}
	{"cpu": 8, "memory": 61000, "storage": 6000, "price": 1470},
	{"cpu": 8, "memory": 68400, "storage": 2000, "price": 1301},
	\end{verbatim}
	
	\item[Type $2$ symmetry] For VMs having the same type, the variables modeling \emph{$vmType_k$} are indistinguishable. Symmetry breakers are the following:
	\begin{alignat*}{2}
	& \left (vmType_{k} = vmType_{k+1} \right) \Longrightarrow \emph{vm}_k^{HR_{t}} = \emph{vm}_{k+1}^{HR_{t}} , & &\quad \text{for all } k=\overline{1,M-1}, \ t=\overline{1,L} \\
	& \left (vmType_{k} = vmType_{k+1} \right) \Longrightarrow \emph{VP}_k = \emph{VP}_{k+1} 
	\end{alignat*}
\end{description}
Now consider the decision variable $A$.  
\begin{description}
	\item[Type $3$ symmetry] For any two or more VMs having the same type, any permutation of the components assigned to these VMs is a solution. 
\end{description}

Type $3$ symmetry is very \textcolor{red}{why so hard} to break. One can reduce some of such symmetries by stating that whenever two consecutive VMs have the same type one of
them must have at least as many components assigned as the other:
\begin{alignat*}{2}
& \left (vmType_{k} = vmType_{k+1} \right) \Longrightarrow \sum_{i=1}^{N}{a_{ik}}  \ge \sum_{i=1}^{N}{a_{i{k+1}}}, \quad k=\overline{1,M-1}
\end{alignat*}
Moreover, we can also impose, for VMs of the same type, a lexicographic order on the respective columns of the assignment matrix $a$
\begin{alignat*}{2}
& \left (vmType_{k} = vmType_{k+1} \right) \Longrightarrow a_{ik}  \prec_{lex} a_{i{k+1}}, \quad k=\overline{1,M-1}, \ i=\overline{1,N}
\end{alignat*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% sec: Row symmetries %%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Row symmetries }\label{sec:rowsym}
